Contribution of ALEGRO to the Update of the European Strategy on Particle Physics

Advanced and novel accelerators (ANAs), driven a by laser pulse or a relativistic particle bunch, have made remarkable progress over the last decades. They accelerated electrons by 10GeV in 30cm (laser driven) and by 42GeV in 85cm (particle bunch driven). Rapid progress continues with lasers, plasma sources, computational methods, and more. In this document we highlight the main contributions made by the various major collaborations, facilities, and experiments that develop ANAs for applications to particle and high-energy physics. These include: ALiVE, ANL-AWA, AWAKE, BNL-ATF, CEPC Injector, DESY-KALDERA, ELI ERIC, EuPRAXIA, HALHF, LBNL-BELLA, LBNL-kBELLA, LCvison, PETRA IV Injector, 10TeV Collider design, SLAC-FACET II, as well as the development of structures, lasers and plasma sources, and sustainability, and demonstrate the intense activities in the field. ANAs can have, and already have, applications to particle and high-energy physics as subsystems, the so-called intermediate applications: injectors, lower energy experiments, beam dump experiments, test beds for detectors, etc. Additionally, an ANA could be an upgrade for any Higgs factory based on a linear accelerator, as proposed in the LCvison project. ANAs have advantages over other concepts for reaching multi-TeV energies: lower geographical and environmental footprints, higher luminosity to power ratio, and are thus more sustainable than other accelerators. However, ANAs must still meet a number of challenges before they can produce bunches with parameters and the luminosity required for a linear collider at the energy frontier. It is therefore extremely important to strongly support vigorous R&D of ANAs, because they are, at this time, the most sustainable acceleration scheme to reach very high energies with a linear accelerator.

==> sections/exec.tex <==
Advanced and novel accelerators (ANAs), driven by a laser pulse or a relativistic particle bunch, have made remarkable progress over the last decades. %
They accelerated electrons by 10\,GeV in 30\,cm (laser driven) and by  42\,GeV in 85\,cm (particle bunch driven). %
Rapid progress continues with lasers, plasma sources, computational methods, and more. %
In this contribution we highlight %progress that was made since the last ESPP, as well as 
the contributions of the various major collaborations, facilities, and experiments that develop ANAs for applications to particle physics and high-energy physics. % 
These include: ALiVE, ANL-AWA, AWAKE, BNL-ATF, CEPC Injector, DESY-kaldera, ELI ERIC, EuPRAXIA, HALHF, LBNL-BELLA, LBNL-kBELLA, LCvison, PETRA IV Injector, 10\,TeV Collider design, SLAC-FACET II, structures, lasers and plasma sources development, and sustainability, and demonstrate the intense activities in the field. %

ANAs can have, and already have, applications to particle and high-energy physics as subsystems, the so-called intermediate applications:
injectors, lower energy experiments, beam dump experiments, test beds for detectors, etc. %
Additionally, an ANA could be an upgrade for any Higgs factory based on a linear accelerator, as proposed in the LCvison project and the 10\,TeV wakefield collider design study. %
ANAs have advantages over other concepts for reaching multi-TeV energies: lower geographical and environmental footprints, higher luminosity to power ratio, and are thus more sustainable than other accelerators. %concepts. %

However, ANAs must still meet a number of challenges before they can produce bunches with parameters and the luminosity required for a linear collider at the energy frontier. %

It is therefore extremely important to strongly support vigorous R\&D of ANAs, because they are, at this time, \emph{the most sustainable acceleration scheme to reach very high energies with a linear accelerator}. %
They also have numerous lower energy applications as light and particle sources for research, industrial, medical, and security applications. %

%Also, no scheme has yet been found to accelerate positron bunches in plasma with quality comparable to that of electrons bunches. % 


==> sections/introduction.tex <==
Wakefield accelerator are structure-based or plasma-based accelerators driven by a laser pulse or a relativistic particle bunch. %
Large fields can be reached in structures (dielectric or metallic) because the wakefield excitation time is shorter than with microwave sources. %
Plasma is a ''broken-down'' gas whose weakly-bound electrons are already ionized, and can thus sustain extremely large fields before further ionization. %

The general goal with wakefield accelerators is to reach average accelerating gradients approaching or exceeding 1\,GeV/m. %
Experiments with dielectric structures driven by a short electron bunch have shown breakdown only at field values exceeding $\approx$14\,GV/m~\cite{dielectric}. %
Driving an 85\,cm-long plasma with the same electron bunch led to the acceleration of 42\,GeV electrons to 84\,GeV~\cite{Blumenfeld}, i.e., with a 52\,GeV/m accelerating gradient. %
Acceleration up to 10\,GeV in a 30\,cm-long plasma channel was recently obtained~\cite{texas,picksley}. %

Plasma sources provide a guiding structure for the drive laser pulse so it can excite wakefields over many Rayleigh lengths of the laser beam. %

Density ramps at the entrance and exit of the plasma source provide additional focusing that allows for the matching of the transverse of the accelerated bunch to the strong focusing force of the accelerator plasma. %

Plasma-based accelerators can also be compact sources of electrons, and potentially serve as injector for a high energy accelerator. %
They provide suitable short electron bunches with very low emittance because of the very large fields that extract electrons from the plasma and accelerates them to relativistic energies over a very short distance. %

Plasma lenses are strong beam optics with axi-symmetric fields (unlike magnetic quadrupoles) and focusing gradients exceeding those of magnetic quadruple by orders of magnitude, a key ingredient to keep the length of the section between accelerating plasmas as short as possible to maintain large average gradient.. %

Plasma mirrors allow for in and out-coupling of drive laser pulses ''on a dime'', another key ingredient to maintain large average gradient. %

It was also shown that particle polarization can also be maintained during the acceleration process~\cite{polarizationplasma}. %
